A Comprehensive Framework for Evaluating API-oriented Code Generation in Large Language Models

Large language models (LLMs) like GitHub Copilot and ChatGPT have emerged as powerful tools for code generation, significantly enhancing productivity and accelerating software development. However, existing benchmarks primarily focus on general code generation without considering API-oriented code generation, i.e., generating code that invokes APIs from specific libraries. Given the growing demand for API-oriented code generation, there is a pressing need for a systematic and automated approach to evaluate LLM on API-oriented code generation. To address this gap, we propose AutoAPIEval, a lightweight and automated framework designed to evaluate the capabilities of LLMs in API-oriented code generation. Our framework works with any library that provides API documentation and focuses on two unit tasks: API recommendation and code example generation, along with four metrics to evaluate the generated APIs and code examples, such as the proportion of incorrect API recommendations for Task 1, and the proportion of code examples where no specific API is invoked and uncompilable/unexecutable code examples for Task 2. In addition, we conducted a case study on three LLMs (ChatGPT, MagiCoder, and DeepSeek Coder) and Java Runtime Environment 8 to demonstrate the framework's effectiveness. Our findings reveal substantial variability in LLM performance across tasks, with ChatGPT adhering better to instructions, while sharing similar effectiveness in code example generation with its counterparts (i.e., MagiCoder and DeekSeek Coder). We also identify key factors associated with code quality, such as API popularity and model confidence, and build classifiers that achieve high accuracy in detecting incorrect API recommendations and erroneous code examples. Retrieval-augmented generation enhances the quality of code generated by LLMs, though its effectiveness varies across different LLMs.

==> result_data.tex <==
RQ1
\begin{table*}[]
\begin{tabular}{c|c|cc}
\hline
\multirow{2}{*}{Model} & API Recommendation & \multicolumn{2}{c}{Snippet Recommendation}                   \\ \cline{2-4} 
                       & Non-Existing (\%)  & \multicolumn{1}{c|}{Uncompilable (\%)} & Unrunnable (\%) \\ \hline
MagiCoder              & 85.3\%             & \multicolumn{1}{c|}{89.7\%}              & 91.9\%            \\
DeepSeek Coder         & 82.9\%             & \multicolumn{1}{c|}{88.9\%}              & 91.6\%            \\
ChatGPT                & 57.3\%             & \multicolumn{1}{c|}{73.0\%}              & 79.1\%           \\ \hline
\end{tabular}
\end{table*}


% % \begin{table*}[h]

% % \begin{tabular}{ |c||*{4}{c|} | *{4}{c|}} 
% %  \hline
% %  \backslashbox{Model}{\% by \# recommended} & Existing API & Compilable & Runnable \\
% %  \hline
% %   MagiCoder & 14.7\% & 10.3\% & 8.1\% \\ 
% %  \hline
% %   DeepSeek Coder & 17.1\% & 11.1\% & 8.4\% \\ 
% %  \hline
% %  ChatGPT & 42.7\% & 27.0\% & 20.9\% \\
% %  \hline
% % \end{tabular}

% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}{*}{Model} & \multicolumn{2}{c|}{API Recommendation}                       & \multicolumn{2}{c}{Snippet Recommendation}                   \\ \cline{2-5} 
                       & \multicolumn{1}{c|}{Recommended API (\#)} & Non-Existing (\#) & \multicolumn{1}{c|}{Uncompilable (\#)} & Unrunnable (\#) \\ \hline
MagiCoder              & \multicolumn{1}{c|}{18412}                & 2711              & \multicolumn{1}{c|}{1896}                & 1508              \\
DeepSeek Coder         & \multicolumn{1}{c|}{20687}                & 3552              & \multicolumn{1}{c|}{2296}                & 1738              \\
ChatGPT                & \multicolumn{1}{c|}{11697}                & 4989              & \multicolumn{1}{c|}{3157}                & 2447             \\ \hline
\end{tabular}
\end{table*}
RQ2



RQ3
% \begin{table*}[h]
% \begin{center}
% \begin{tabular}{ *{5}{|c}| } 
% \hline
%  \multicolumn{2}{|c|}{} & Task 1 & \multicolumn{2}{c|}{Task 2} \\
% \hline
% Model & \backslashbox{Temperature}{\% by \# recommended} & Existing API & Compilable & Runnable \\
% \hline
% \multirow{6}{5em}{MagiCoder} & 0 & 14.7\% & 10.3\% & 8.1\% \\ 
% \cline{2-5}
% & 0.2 & 15.2\% & 10.4\% & 8.2\% \\ 
% \cline{2-5}
% & 0.4 & 15.8\% & 10.6\% & 8.3\% \\ 
% \cline{2-5}
% & 0.6 & 15.5\% & 9.9\% & 7.7\% \\ 
% \cline{2-5}
% & 0.8 & 15.4\% & 9.5\% & 7.3\% \\ 
% \cline{2-5}
% & 1.0 & 14.7\% & 8.8\% & 6.9\% \\ 
% \hline
% \multirow{4}{5em}{ChatGPT} & 0 & 42.7\% & 27.0\% & 20.9\% \\ 
% \cline{2-5}
% & 0.4 & 42.2\% & 27.6\% & 21.0\% \\ 
% \cline{2-5}
% & 0.8 & 40.8\% & 26.5\% & 20.4\% \\ 
% \cline{2-5}
% & 1.0 & 39.4\% & 25.2\% & 19.6\% \\ 
% \hline
% \end{tabular}
% \end{center}
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
\caption{}
\begin{tabular}{c|c|c|cc}
\hline
\multirow{2}{*}{Model}     & \multirow{2}{*}{Temperature} & API Recommendation & \multicolumn{2}{c}{Snippet Recommendation}          \\ \cline{3-5} 
                           &                              & Non-Existing (\%)      & \multicolumn{1}{c|}{Uncompilable (\%)} & Unrunnable(\%) \\ \hline
\multirow{6}{*}{MagiCoder} & 0                            & 85.3\%             & \multicolumn{1}{c|}{89.7\%}          & 91.9\%        \\
                           & 0.2                          & 84.8\%             & \multicolumn{1}{c|}{89.6\%}          & 91.8\%        \\
                           & 0.4                          & 84.2\%             & \multicolumn{1}{c|}{80.4\%}          & 91.7\%        \\
                           & 0.6                          & 84.5\%             & \multicolumn{1}{c|}{90.1\%}           & 92.3\%        \\
                           & 0.8                          & 84.6\%             & \multicolumn{1}{c|}{90.5\%}           & 92.7\%        \\
                           & 1.0                          & 85.3\%             & \multicolumn{1}{c|}{91.2\%}           & 93.1\%        \\ \cline{1-1}
\multirow{4}{*}{ChatGPT}   & 0                            & 57.3\%             & \multicolumn{1}{c|}{73.0\%}          & 79.1\%       \\
                           & 0.4                          & 57.8\%             & \multicolumn{1}{c|}{72.4\%}          & 79.0\%       \\
                           & 0.8                          & 59.2\%             & \multicolumn{1}{c|}{73.5\%}          & 79.6\%       \\
                           & 1.0                          & 60.6\%             & \multicolumn{1}{c|}{74.8\%}          & 80.4\%       \\ \hline
\end{tabular}
\end{table*}


RQ4

Random Forest Classifier

\begin{table*}[h]
\caption{MagiCoder Task 1 Random Forest Classifier}
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Method Exist} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c}{Support} \\ \hline
\multicolumn{1}{c|}{False}        & \multicolumn{1}{c|}{0.95}      & \multicolumn{1}{c|}{0.98}   & \multicolumn{1}{c|}{0.96}     & \multicolumn{1}{c}{18850}   \\
\multicolumn{1}{c|}{True}         & \multicolumn{1}{c|}{0.65}      & \multicolumn{1}{c|}{0.4}    & \multicolumn{1}{c|}{0.49}     & \multicolumn{1}{c}{1696}    \\
\multicolumn{1}{c|}{accuracy}     & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{0.93}     & \multicolumn{1}{c}{20546}   \\
\multicolumn{1}{c|}{macro avg}    & \multicolumn{1}{c|}{0.80}      & \multicolumn{1}{c|}{0.69}   & \multicolumn{1}{c|}{0.73}     & \multicolumn{1}{c}{20546}   \\
\multicolumn{1}{c|}{weighted avg} & \multicolumn{1}{c|}{0.92}      & \multicolumn{1}{c|}{0.93}   & \multicolumn{1}{c|}{0.92}     & \multicolumn{1}{c}{20546}   \\ \hline
                                  &                                &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{Indicator}    & Feature Importance             &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{API Length}   & 0.1852                         &                             &                               &                             \\
\multicolumn{1}{l|}{Confidence}   & 0.2364                         &                             &                               &                             \\
\multicolumn{1}{l|}{PPL}          & 0.3158                         &                             &                               &                             \\
\multicolumn{1}{l|}{Popularity}   & 0.2626                         &                             &                               &          \\  \cline{1-2}                   
\end{tabular}
\end{table*}

\begin{table*}[]
\caption{MagiCoder Task 2 Random Forest Classifier}
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Snippet Runnable} & Precision                 & Recall                    & \multicolumn{1}{c|}{F1-score} & Support \\ \hline
\multicolumn{1}{c|}{False}            & \multicolumn{1}{c|}{0.77} & \multicolumn{1}{c|}{0.76} & \multicolumn{1}{c|}{0.77}     & 261     \\
\multicolumn{1}{c|}{True}             & \multicolumn{1}{c|}{0.67} & \multicolumn{1}{c|}{0.67} & \multicolumn{1}{c|}{0.67}     & 184     \\
\multicolumn{1}{c|}{accuracy}         & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{0.73}     & 445     \\
\multicolumn{1}{c|}{macro avg}        & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{0.72}     & 445     \\
\multicolumn{1}{c|}{weighted avg}     & \multicolumn{1}{c|}{0.73} & \multicolumn{1}{c|}{0.73} & \multicolumn{1}{c|}{0.73}     & 445     \\ \hline
                                      &                           &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Indicator}        & Feature Importance        &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Mean Dist}        & 0.3431                    &                           &                               &         \\
\multicolumn{1}{c|}{Max Dist}         & 0.3681                    &                           &                               &         \\
\multicolumn{1}{c|}{Popularity}       & 0.2888                    &                           &                               &         \\  \cline{1-2}
\end{tabular}
\end{table*}



\begin{table*}[]
\caption{ChatGPT Task 1 Random Forest Classifier}
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Method Exist} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c}{Support} \\ \hline
\multicolumn{1}{c|}{False}        & \multicolumn{1}{c|}{0.87}      & \multicolumn{1}{c|}{0.92}   & \multicolumn{1}{c|}{0.90}     & \multicolumn{1}{c}{6775}    \\
\multicolumn{1}{c|}{True}         & \multicolumn{1}{c|}{0.68}      & \multicolumn{1}{c|}{0.55}   & \multicolumn{1}{c|}{0.61}     & \multicolumn{1}{c}{2071}    \\
\multicolumn{1}{c|}{accuracy}     & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{0.83}     & \multicolumn{1}{c}{8846}    \\
\multicolumn{1}{c|}{macro avg}    & \multicolumn{1}{c|}{0.78}      & \multicolumn{1}{c|}{0.73}   & \multicolumn{1}{c|}{0.75}     & \multicolumn{1}{c}{8846}    \\
\multicolumn{1}{c|}{weighted avg} & \multicolumn{1}{c|}{0.83}      & \multicolumn{1}{c|}{0.83}   & \multicolumn{1}{c|}{0.83}     & \multicolumn{1}{c}{8846}    \\ \hline
                                  &                                &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{Indicator}    & Feature Importance             &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{API Length}   & 0.1932                         &                             &                               &                             \\
\multicolumn{1}{l|}{Confidence}   & 0.2704                         &                             &                               &                             \\
\multicolumn{1}{l|}{PPL}          & 0.2612                         &                             &                               &                             \\
\multicolumn{1}{l|}{Popularity}   & 0.2751                         &                             &                               &         \\  \cline{1-2}          
\end{tabular}
\end{table*}

\begin{table*}[]
\caption{ChatGPT Task 2 Random Forest Classifier}
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Snippet Runnable} & Precision                 & Recall                    & \multicolumn{1}{c|}{F1-score} & Support \\ \hline
\multicolumn{1}{c|}{False}            & \multicolumn{1}{c|}{0.65} & \multicolumn{1}{c|}{0.57} & \multicolumn{1}{c|}{0.61}     & 190     \\
\multicolumn{1}{c|}{True}             & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{0.78} & \multicolumn{1}{c|}{0.75}     & 272     \\
\multicolumn{1}{c|}{accuracy}         & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{0.69}     & 462     \\
\multicolumn{1}{c|}{macro avg}        & \multicolumn{1}{c|}{0.68} & \multicolumn{1}{c|}{0.68} & \multicolumn{1}{c|}{0.68}     & 462     \\
\multicolumn{1}{c|}{weighted avg}     & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{0.69}     & 462     \\ \hline
                                      &                           &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Indicator}        & Feature Importance        &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Mean Dist}        & 0.3411                    &                           &                               &         \\
\multicolumn{1}{c|}{Max Dist}         & 0.3433                    &                           &                               &         \\
\multicolumn{1}{c|}{Popularity}       & 0.3155                    &                           &                               &         \\  \cline{1-2}
\end{tabular}
\end{table*}

RQ5


% \begin{table*}[]
% \caption{RAG}
% \centering
% \begin{tabular}{c|c|cc}
% \hline
% \multirow{2}{*}{Model} & API Recommendation & \multicolumn{2}{c}{Snippet Recommendation}           \\ \cline{2-4} 
%                        & Existing (\%)      & \multicolumn{1}{c|}{Compilable (\%)} & Runnable (\%) \\ \hline
% MagiCoder (w/o retrieval)              & 14.7\%             & \multicolumn{1}{c|}{10.3\%} ()        & 8.1\%         \\
% MagiCoder (w/ retrieval)     & 16.0\% ($1.3\%\uparrow$)              & \multicolumn{1}{c|}{11.3\% ($1.0\%\uparrow$)  }        & 9.0\% ($0.9\%\uparrow$)         \\
% ChatGPT  (w/o retrieval)              & 42.7\%             & \multicolumn{1}{c|}{27.0\%}          & 20.9\%        \\
% ChatCPT (w/ retrieval)       & 45.7\% ($3.0\%\uparrow$)            & \multicolumn{1}{c|}{28.5\% ($1.5\%\uparrow$)}          & 21.7\% ($0.8\%\uparrow$)       \\ \hline
% \end{tabular}
% \end{table*}

\begin{table}[]
\begin{tabular}{c|c|cc}
\hline
\multirow{2}{*}{Model} & API Recommendation & \multicolumn{2}{c}{Snippet Recommendation}                   \\ \cline{2-4} 
                       & Non-Existing (\%)  & \multicolumn{1}{c|}{Uncompilable (\%)}   & Unrunnable (\%) \\ \hline
MagiCoder              & 85.3\%             & \multicolumn{1}{c|}{89.7\%}              & 91.9\%            \\
MagiCoder with RAG     & 84.0\%             & \multicolumn{1}{c|}{88.7\%}              & 91.0\%            \\
ChatGPT                & 57.3\%             & \multicolumn{1}{c|}{73.0\%}              & 79.1\%            \\
ChatCPT with RAG       & 54.3\%             & \multicolumn{1}{c|}{71.5\%}              & 79.3\%            \\ \hline
\end{tabular}
\end{table}

% redundant

==> rq2_old.tex <==
\subsection{Results of RQ2}\label{sec:rq2}

% \begin{figure}
% \centering
% \includegraphics[scale=0.62]{RQ2-result.png}
% \caption{RQ2 Data Table}
% \label{rq2-data-result}
% \end{figure}

\begin{figure}
\centering
\resizebox{\columnwidth}{!}{
    \includegraphics[scale=1]{result data figures/rq2/Hallucination Types.png}
}
\caption{RQ2 Hallucination Type}
\label{rq2-hallucination-type}
\end{figure}



\begin{table*}[]
\centering
\caption{Frequency of each type of errors for API recommendation and code example generation. }
\begin{tabular}{cc|cc|cc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Types}}                                                                    & \multicolumn{2}{c|}{MagiCoder}       & \multicolumn{2}{c}{ChatGPT}          \\ \cline{3-6} 
\multicolumn{2}{c|}{}                                                                                          & \multicolumn{1}{c|}{Task 1} & Task 2 & \multicolumn{1}{c|}{Task 1} & Task 2 \\ \hline
\multicolumn{2}{c|}{Factual Fabrication}                                                                       & \multicolumn{1}{c|}{180}    & 52     & \multicolumn{1}{c|}{197}    & 46     \\
\multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Factual Inconsistency,  Parameter Inconsistency\end{tabular}} & \multicolumn{1}{c|}{89}     & 55     & \multicolumn{1}{c|}{66}     & 42     \\
\multicolumn{2}{c|}{Instruction Inconsistency}                                                                 & \multicolumn{1}{c|}{115}    & 21     & \multicolumn{1}{c|}{121}    & 6      \\
\multicolumn{2}{c|}{Context Inconsistency}                                                                     & \multicolumn{1}{c|}{}       & 6      & \multicolumn{1}{c|}{}       &        \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{Logical Inconsistency}}           & Context Preparation Error              & \multicolumn{1}{c|}{}       & 39     & \multicolumn{1}{c|}{}       & 98     \\
\multicolumn{1}{c|}{}                                                 & Exception Handling                     & \multicolumn{1}{c|}{}       & 22     & \multicolumn{1}{c|}{}       & 20     \\
\multicolumn{1}{c|}{}                                                 & Missing Import Statement               & \multicolumn{1}{c|}{}       & 19     & \multicolumn{1}{c|}{}       & 32     \\
\multicolumn{1}{c|}{}                                                 & API Knowledge Error                    & \multicolumn{1}{c|}{}       & 21     & \multicolumn{1}{c|}{}       & 10     \\
\multicolumn{1}{c|}{}                                                 & Type Mismatch                          & \multicolumn{1}{c|}{}       & 21     & \multicolumn{1}{c|}{}       & 9      \\
\multicolumn{1}{c|}{}                                                 & Polymorphism Error                     & \multicolumn{1}{c|}{}       & 22     & \multicolumn{1}{c|}{}       & 16     \\ \hline
\multicolumn{1}{c|}{\multirow{7}{*}{Other}}                           & UI Initiation Error                    & \multicolumn{1}{c|}{}       & 35     & \multicolumn{1}{c|}{}       & 58     \\
\multicolumn{1}{c|}{}                                                 & Timeout Error                          & \multicolumn{1}{c|}{}       & 11     & \multicolumn{1}{c|}{}       & 1      \\
\multicolumn{1}{c|}{}                                                 & Connection Required                    & \multicolumn{1}{c|}{}       & 16     & \multicolumn{1}{c|}{}       & 3      \\
\multicolumn{1}{c|}{}                                                 & External Resource Required             & \multicolumn{1}{c|}{}       & 25     & \multicolumn{1}{c|}{}       & 20     \\
\multicolumn{1}{c|}{}                                                 & Pre-Assumption Error                   & \multicolumn{1}{c|}{}       & 3      & \multicolumn{1}{c|}{}       & 0      \\
\multicolumn{1}{c|}{}                                                 & Deprecated Error                       & \multicolumn{1}{c|}{}       & 9      & \multicolumn{1}{c|}{}       & 23     \\
\multicolumn{1}{c|}{}                                                 & Incomplete Code Snippet Error          & \multicolumn{1}{c|}{}       & 7      & \multicolumn{1}{c|}{}       & 0      \\ \hline
\end{tabular}
\end{table*}


% \begin{figure}
% \centering
% \includegraphics[scale=0.52]{RQ2-other.png}
% \caption{RQ2 "Other" error}
% \label{rq2-other}
% \end{figure}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=RQ2 "Other" error,
    label=rq2-other
]
import java.util.Scanner;

public class Scanner_4 {
    public static void main(String[] args) {
        Scanner scanner = new Scanner(System.in);
        System.out.println("Enter a double:");
        double input = scanner.nextDouble();
        System.out.println("You entered: " + input);
    }
}
\end{lstlisting}

Listing~\ref{rq2-fabrication-recommendation} is an example of Factual Fabrication from code recommendation. As we can see, none of the methods recommended actually exist in the "java.util.Arrays" package, they are method from the class "java.util.ArrayList". We are not sure if the similarity in the package name (Arrays vs ArrayList) confuses the LLM. Or the example "boolean add(E e)" confuses the LLM because it the package ArrayList also contains this method.

% \begin{figure}
% \centering
% \includegraphics[scale=0.5]{RQ2-Factual-Fabrication-In-Recommendation.png}
% \caption{RQ2 "Factual Fabrication" In Code Recommendation}
% \label{rq2-fabrication-recommendation}
% \end{figure}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    caption=RQ2 "Factual Fabrication" In Code Recommendation,
    label=rq2-fabrication-recommendation
]
/*
@@ Instruction
I want to use java.util.Arrays package from Java
recommend a list of useful with at most 5 apis for this package, exlclude method inherent from its parent class
For each api method specify its return type and parameters in the below format

format: return_type method_name()

For example:
`boolean add(E e)`: This method appends the specified element to the end of this list.
*/
@@ Response
1. `boolean add(E e)`: This method appends the specified element to the end of this list.
2. `void add(int index, E element)`: This method inserts the specified element at the specified position in this list.
3. `boolean addAll(Collection<? extends E> c)`: This method appends all of the elements in the specified collection to the end of this list, in the order that they are returned by the specified collection`s iterator.
4. `boolean addAll(int index, Collection<? extends E> c)`: This method inserts all of the elements in the specified collection into this list, starting at the specified position.
5. `void clear()`: This method removes all of the elements from this list.

\end{lstlisting}

Listing~\ref{rq2-fabrication-generation} is an example of Factual Fabrication from code generation. As we can see, there is an error saying that the method "createCompatibleGraphics()" method does not exist. And if you are curious, the method that exists is actually called "createCompatibleImage()".

% \begin{figure}
% \centering
% \includegraphics[scale=0.45]{RQ2-Factual-Fabrication-In-Generation.png}
% \caption{RQ2 "Factual Fabrication" In Code Generation}
% \label{rq2-fabrication-generation}
% \end{figure}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=RQ2 "Factual Fabrication" In Code Generation,
    label=rq2-fabrication-generation,
    breaklines=true,
    breakatwhitespace=false
]
import java.awt.Font;
import java.awt.FontMetrics;
import java.awt.Graphics;
import java.awt.GraphicsEnvironment;

public class FontMetrics_3 {
    public static void main(String[] args) {
        GraphicsEnvironment ge = GraphicsEnvironment.getLocalGraphicsEnvironment();
        Graphics g = ge.getDefaultScreenDevice().getDefaultConfiguration().createCompatibleGraphics(null);
        Font font = new Font("Arial", Font.PLAIN, 12);
        g.setFont(font);
        FontMetrics fm = g.getFontMetrics();
        int height = fm.getHeight();
        System.out.println("Height of the font in pixels: " + height);
    }
}

/*
output:
./java_awt/javaFiles/FontMetrics_3.java:9: error: cannot find symbol
        Graphics g = ge.getDefaultScreenDevice().getDefaultConfiguration().createCompatibleGraphics(null);
             ^
  symbol:   method createCompatibleGraphics(<null>)
  location: class GraphicsConfiguration
1 error
*/
\end{lstlisting}

For Factual Inconsistency, Parameter Inconsistency. It happens when only the signature of method is wrong. This mostly appears in the code recommendation task, consisting 26.25\% of the error from Task 1. Figure~\ref{rq2-inconsistency-recommendation} shows the response from LLM when asked to recommend method for the class "java.util.Base64". Only the recommended method from number 1 to 6 actually exist. All the methods recommended starting from 7 have incorrect method signature.

% \begin{figure}
% \centering
% \includegraphics[scale=0.46]{RQ2-Factual-Inconsistency-In-Recommendation.png}
% \caption{RQ2 "Factual Inconsistency" In Code Recommendation}
% \label{rq2-inconsistency-recommendation}
% \end{figure}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    caption=RQ2 "Factual Inconsistency" In Code Recommendation,
    label=rq2-inconsistency-recommendation
]
/*
@@ Response
Here is a list of useful methods from the `java.util.Base64` package:
*/
1. `static byte[] getDecoder()`: Returns a Base64.Decoder that converts the Base64 data to a byte array.
2. `static byte[] getEncoder()`: Returns a Base64.Encoder that converts a byte array to Base64 data.
3. `static byte[] decode(byte[] src)`: Decodes the specified byte array into a new byte array.
4. `static byte[] decode(String src)`: Decodes the specified String into a new byte array.
5. `static byte[] encode(byte[] src)`: Encodes the specified byte array into a new byte array.
6. `static String encodeToString(byte[] src)`: Encodes the specified byte array into a String.
7. `static String encodeToString(String src)`: Encodes the specified String into a String.
8. `static String encodeToString(byte[] src, int off, int len)`: Encodes the specified byte array into a String.
9. `static String encode(byte[] src, int off, int len)`: Encodes the specified byte array into a new byte array.
10. `static byte[] decode(String src, int off, int len)`: Decodes the specified String into a new byte array.
11. `static byte[] decode(byte[] src, int off, int len)`: Decodes the specified byte array into a new byte array.
12. `static byte[] decode(String src, Base64.Decoder decoder)`: Decodes the specified String using the specified Decoder.
13. `static byte[] decode(byte[] src, Base64.Decoder decoder)`: Decodes the specified byte array using the specified Decoder.
...

\end{lstlisting}

Although it is very rare, this can also happen in the generated code when the code is using the correct method name but with wrong parameter(s).

Listing~\ref{rq2-inconsistency-generation} is an example for Factual Inconsistency in code generation. As we can see, the parameter provided for the constructor method is not correct, thus causing the error.

% \begin{figure}
% \centering
% \includegraphics[scale=0.45]{RQ2-Factual-Inconsistency-In-Generation.png}
% \caption{RQ2 "Factual Inconsistency" In Code Generation}
% \label{rq2-inconsistency-generation}
% \end{figure}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=RQ2 "Factual Inconsistency" In Code Generation,
    label=rq2-inconsistency-generation,
    breaklines=true,
    breakatwhitespace=false
]
import javax.management.MBeanParameterInfo;

public class MBeanParameterInfo_2 {
    public static void main(String[] args) {
        MBeanParameterInfo parameterInfo = new MBeanParameterInfo("name", "type", "description", false, false);
        String type = parameterInfo.getType();
        System.out.println("Type of the parameter: " + type);
    }
}

/*
output:
./javax_management/javaFiles/MBeanParameterInfo_2.java:5: error: no suitable constructor found for MBeanParameterInfo(String,String,String,boolean,boolean)
        MBeanParameterInfo parameterInfo = new MBeanParameterInfo("name", "type", "description", false, false);

    constructor MBeanParameterInfo.MBeanParameterInfo(String,String,String) is not applicable
      (actual and formal argument lists differ in length)
    constructor MBeanParameterInfo.MBeanParameterInfo(String,String,String,Descriptor) is not applicable
      (actual and formal argument lists differ in length)
1 error
*/
\end{lstlisting}

For Instruction Inconsistency, it happens when the LLM does not follow our format for recommending the method. For example, the LLM tends to ignore and not output the return type of a method if the return type is "void". For some of the static method, the LLM would also ignore the return type and output the method as "Class.method" format. This format is how the method should be called in the actual code snippet, instead of listing the method like you would see in a documentation.

Logical Inconsistency only happen in Task 2, when the generated code snippet has logical error and resulting in a failure execution of the code. The causes logical error from the code varies greatly. Sometimes the LLM pass null as a method parameter when it should have not done so. Sometimes the LLM put try catch block around the code when the code does not throw exception. Sometimes the LLM catch the wrong exception. Listing~\ref{rq2-logical-inconsistency} shows one kind of the error, It is trying to catch IOException when this exception would never be thrown in the code.

% \begin{figure}
% \centering
% \includegraphics[scale=0.5]{RQ2-Logical-Inconsistency.png}
% \caption{RQ2 "Logical Inconsistency"}
% \label{rq2-logical-inconsistency}
% \end{figure}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=RQ2 "Logical Inconsistency,
    label=rq2-logical-inconsistency,
    breaklines=true,
    breakatwhitespace=false
]
import java.io.ByteArrayOutputStream;
import java.io.IOException;

public class ByteArrayOutputStream_1 {
    public static void main(String[] args) {
        ByteArrayOutputStream baos = new ByteArrayOutputStream();
        try {
            baos.write(1);
            baos.write(2);
            baos.write(3);
        } catch (IOException e) {
            e.printStackTrace();
        }
        System.out.println("Size of ByteArrayOutputStream: " + baos.size());
    }
}

/*
output:
./java_io/javaFiles/ByteArrayOutputStream_1.java:11: error: exception IOException is never thrown in body of corresponding try statement
        } catch (IOException e) {
          ^
1 error
*/
\end{lstlisting}

The result of RQ2 shows us that the LLM can be wrong in so many ways when performing Code Recommendation/Generation task. There are many cases that the hallucination is built on some truthful knowledge, but with a small error lying in the response somewhere. For people who do not have domain knowledge, these small errors can be great obstacles if they are trying to learn something new by asking the LLM. The influence of hallucination from LLM cannot be underestimated.

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=Context Preparation Error Example
]
import java.awt.event.MouseEvent;

public class MouseEvent_3 {
    public static void main(String[] args) {
        MouseEvent event = new MouseEvent(null, 0, 0, 0, 0, 0, 0, false, 0);
        int clickCount = event.getClickCount();
        System.out.println("Number of times the mouse button has been clicked: " + clickCount);
    }
}
\end{lstlisting}


\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=Exception Handling Error Example
]
import java.awt.Desktop;
import java.net.URI;
import java.net.URISyntaxException;

public class Desktop_2 {
    public static void main(String[] args) {
        try {
            Desktop desktop = Desktop.getDesktop();
            URI uri = new URI("http://www.google.com");
            desktop.browse(uri);
        } catch (URISyntaxException | java.awt.AWTException e) {
            e.printStackTrace();
        }
    }
}
/*
output:
./java_awt/javaFiles/Desktop_2.java:11: error: exception AWTException is never thrown in body of corresponding try statement
        } catch (URISyntaxException | java.awt.AWTException e) {
                                              ^
./java_awt/javaFiles/Desktop_2.java:10: error: unreported exception IOException; must be caught or declared to be thrown
            desktop.browse(uri);
*/
\end{lstlisting}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=Missing Import Statement Error Example
]
import java.text.Format;

public class Format_1 {
    public static void main(String[] args) {
        Format f = new Format() {
            @Override
            public StringBuffer format(Object obj, StringBuffer toAppendTo, FieldPosition pos) {
                return toAppendTo.append(obj.toString());
            }

            @Override
            public Object parseObject(String source, ParsePosition pos) {
                return null;
            }
        };

        String str = f.format("Hello, World!");
        System.out.println(str);
    }
}

/*
output:
./java_text/javaFiles/Format_1.java:7: error: cannot find symbol
            public StringBuffer format(Object obj, StringBuffer toAppendTo, FieldPosition pos) {

  symbol: class FieldPosition
./java_text/javaFiles/Format_1.java:12: error: cannot find symbol
            public Object parseObject(String source, ParsePosition pos) {

  symbol: class ParsePosition
*/
\end{lstlisting}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=API Knowledge Error Example
]
import java.util.UUID;

public class UUID_1 {
    public static void main(String[] args) {
        String name = "6ec0c9f0-755e-4287-9a51-a2c31exxxxx";
        UUID uuid = UUID.fromString(name);
        System.out.println(uuid);
    }
}

/*
output:
stderr:
Exception in thread "main" java.lang.NumberFormatException: Error at index 6 in: "a2c31exxxxx"
	at java.base/java.lang.NumberFormatException.
 forCharSequence(NumberFormatException.java:83)
	at java.base/java.lang.Long.parseLong(Long.java:794)
	at java.base/java.util.UUID.fromString1(UUID.java:290)
	at java.base/java.util.UUID.fromString(UUID.java:258)
	at UUID_1.main(UUID_1.java:6)
*/
\end{lstlisting}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=Type Mismatch
]
import java.awt.geom.QuadCurve2D;

public class QuadCurve2D_Float_4 {
    public static void main(String[] args) {
        QuadCurve2D.Float curve = new QuadCurve2D.Float(0, 0, 10, 10, 20, 20);
        float y1 = curve.getY1();
        System.out.println("Y1: " + y1);
    }
}

/*
output:
./java_awt_geom/javaFiles/QuadCurve2D_Float_4.java:6: error: incompatible types: possible lossy conversion from double to float
        float y1 = curve.getY1();
                              ^
1 error
*/
\end{lstlisting}

\begin{lstlisting}[
    float,
    basicstyle=\small,
    language=Java,
    caption=Polymorphism Error
]
import java.net.CacheRequest;

public class CacheRequest_4 {
    public static void main(String[] args) {
        CacheRequest request = new CacheRequest() {
            @Override
            public void abort() {
                // Implementation of abort method
            }
        };

        // Call the abort method
        request.abort();
    }
}

/*
output:
./java_net/javaFiles/CacheRequest_4.java:5: error: <anonymous CacheRequest_4$1> is not abstract and does not override abstract method getBody() in CacheRequest
        CacheRequest request = new CacheRequest() {
                                                  ^
1 error
*/

\end{lstlisting}



==> rq3.tex <==
\subsection{RQ3 - Model Setting Analysis}\label{sec:rq3}
%\yt{how many times do you attempt? This is a very surprising finding, but it seems to conflict with Table 5, which shows that the middle value is better. Are the differences significant?}\sw{typo, higher temperature tends to produce more error and lower quality recommendation.}
\textbf{In general, using a lower temperature tends to produce code of similar or higher quality for both tasks.} Figure~\ref{fig:temperature} presents the quality of code generation for both tasks under different temperatures. For Task 1, we observe that for ChatGPT, the \NoneExistP value increases from 57.3\% to 60.6\% as the temperature rises. However, for MagiCoder, \NoneExistP remains consistent regardless of temperature. In Task 2, MagiCoder's \total improves from 44.4\% to 53.1\% as the temperature increases from 0 to 1, while ChatGPT's proportion of total erroneous code examples remains stable, fluctuating slightly between 50.1\% and 51.0\%.

%the value of \NoneExistP increases from 57.3\% to 60.6\% as the temperature increases. For MagiCoder, \NoneExistP remains stable when temperature increases. In Task 2, for MagiCoder, \total increases from 44.4\% to 53.1\% as the temperature rise from 0 to 1. For ChatGPT, the proportion of total erroneous code examples remains relatively stable, ranging from 50.1\% to 51.0\%. 

\begin{figure}[h]
\centering

  \includegraphics[width=0.8\textwidth]{figures/PDPChatgptTask1.pdf}
  \vspace{-0.3cm}
\caption{The impact of temperature on the quality of AIP-oriented code generation.}
\label{fig:temperature}
\end{figure}

\textbf{The studied three decoding strategies share similar performance in API recommendation and code example generation.} Table~\ref{tab:rq3-decoding} presents the comparison between different decoding strategies on Task 1 and Task 2 when using MagiCoder. As we can see, Greedy Search (84.6\%) achieves a slightly lower proportion of incorrect API, compared with Beam Search (86.7\%) and Top K (85.3\%). For Task 2, Top K achieves a slightly lower \total compared with the other two decoding strategies. In general, all three decoding strategies share similar performance. 


\begin{table}[h]
\caption{The impact of decoding strategy on the quality of code generation.}\label{tab:rq3-decoding}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|l|l|l|l|l|l}
\hline
\multirow{2}{*}{\textbf{Model}}     & \multirow{2}{*}{\textbf{Decoding Strategy}} & \textbf{Task 1} & \multicolumn{4}{c}{\textbf{Task 2}}                                                       \\ \cline{3-7} 
                           &                                    & \textbf{\NoneExistP}   & \textbf{\NoAPIUsedP} & \textbf{\UnCompilableP} & \textbf{\NonRunnableP} & \textbf{\total}\\ \hline
\multirow{3}{*}{MagiCoder} & Greedy Search                      & \textbf{84.6\%} (15,055/17,789)            & 10.4\% (283/2,734)          & 20.1\% (550/2,734)            & 15.5\% (420/2,734)  & 45.8\% (1,253/2,734)       \\
                           & Beam Search                        & 86.7\% (28,618/33,012)            & \textbf{5.7\%} (251/4,394)          & 21.7\% (953/4,394)            & 19.4\% (854/4,394)  & 46.8\% (2,058/4,394)       \\
                           & Top K (k=5)                        & 85.3\% (15,701/18,412)            & 9.1\% (247/2,711)          & \textbf{21.0\%} (568/2,711)            & \textbf{14.3\%} (388/2,711)   &  \textbf{44.3\%} (1,203/2,711)       \\ \hline
\end{tabular}
}
\end{table}


\rqboxc{In general, a lower temperature tends to produce code of similar or higher quality for both tasks and across both LLMs. Greedy Search, Beam Search, and Top-K share similar performance.}

% \begin{table}[]
% \caption{Decoding Strategy without uncompilable}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|c|c|cc}
% \hline
% \multirow{2}{*}{Model}     & \multirow{2}{*}{Decoding Strategy} & API Recommendation & \multicolumn{2}{c}{Snippet Recommendation}              \\ \cline{3-5} 
%                            &                                    & \NoneExistP (\%)    & \multicolumn{1}{c|}{\NoAPIUsedP (\%)} & \NonRunnableP(\%) \\ \hline
% \multirow{3}{*}{MagiCoder} & Greedy Search                      & 84.6\%             & \multicolumn{1}{c|}{86.2\%}          & 92.0\%           \\
%                            & Beam Search                        & 86.7\%             & \multicolumn{1}{c|}{87.5\%}          & 93.0\%           \\
%                            & Top K (k=5)                        & 85.3\%             & \multicolumn{1}{c|}{86.1\%}          & 91.8\%           \\ \hline
% \end{tabular}
% }
% \end{table}



% \begin{table}[]
% \caption{Top K\sw{where is k=5 for chatgpt?}\yw{we didn't run it}}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|c|c|ccc}
% \hline
% \multirow{2}{*}{\textbf{Model}}   & \multirow{2}{*}{\textbf{TopK}} & \textbf{Task 1} & \multicolumn{3}{c}{\textbf{Task 2}}                                                       \\ \cline{3-6} 
%                          &                       & \textbf{\NoneExistP}   & \multicolumn{1}{c|}{\textbf{\NoAPIUsedP}} & \multicolumn{1}{c|}{\textbf{\UnCompilableP}} & \textbf{\NonRunnableP} \\ \hline
% \multirow{3}{*}{MagiCoder}                & 1                     & 85.2\% (15,451/18,133)            & \multicolumn{1}{c|}{9.6\% (257/2,682)}          & \multicolumn{1}{c|}{21.6\% (580/2,682)}            & 36.4\% (975/2,682)          \\
%                          & 5                     & 85.3\% (15,701/18,412)             & \multicolumn{1}{c|}{9.1\% (247/2,711)}          & \multicolumn{1}{c|}{21.0\% (568/2,711)}            & 35.2\% (956/2,711)           \\
%                          & 10                    & 85.0\% (15,405/18,124)            & \multicolumn{1}{c|}{10.2\% (277/2,719)}          & \multicolumn{1}{c|}{22.1\% (600/2,719)}            & 35.7\% (972/2,719)          \\ \hline
% \multirow{2}{*}{ChatGPT} & 1                     & 57.0\% (6,708/11,764)            & \multicolumn{1}{c|}{2.7\% (135/5,056)}          & \multicolumn{1}{c|}{31.3\% (1,580/5,056)}            & 46.1\% (2,331/5,056)          \\
%                          & 10                    & 57.4\% (6,744/11,758)            & \multicolumn{1}{c|}{2.9\% (144/5,014)}          & \multicolumn{1}{c|}{31.7\% (1,590/5,014)}            & 46.6\% (2,335/5,014)          \\ \hline
% \end{tabular}
% }
% \end{table}

% \begin{table}[]
% \caption{Top K without uncompilable}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{c|c|c|cc}
% \hline
% \multirow{2}{*}{Model}   & \multirow{2}{*}{TopK} & API Recommendation & \multicolumn{2}{c}{Snippet Recommendation}              \\ \cline{3-5} 
%                          &                       & \NoneExistP (\%)    & \multicolumn{1}{c|}{\NoAPIUsedP (\%)} & \NonRunnableP(\%) \\ \hline
% \multirow{3}{*}{MagiCoder}                & 1                     & 85.2\%             & \multicolumn{1}{c|}{86.6\%}          & 92.0\%           \\
%                          & 5                     & 82.3\%             & \multicolumn{1}{c|}{86.1\%}          & 91.8\%           \\
%                          & 10                    & 85.0\%             & \multicolumn{1}{c|}{85.7\%}          & 91.9\%           \\ \hline
% \multirow{2}{*}{ChatGPT} & 1                     & 57.0\%             & \multicolumn{1}{c|}{58.1\%}          & 78.0\%           \\
%                          & 10                    & 57.4\%             & \multicolumn{1}{c|}{58.6\%}          & 78.4\%           \\ \hline
% \end{tabular}
% }
% \end{table}




% \begin{table}[h]
% \caption{The impact of temperature on the quality of API-oriented code generation.}\label{tab:RQ3-temp}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|l|l|l|l|l|l}
% \hline
% \multirow{2}{*}{\textbf{Model}}     & \multirow{2}{*}{\textbf{Temperature}} & \textbf{Task 1}& \multicolumn{4}{c}{\textbf{Task 2}}                                                       \\ \cline{3-7} 
%                            &                              & \textbf{\NoneExistP}    & \textbf{\NoAPIUsedP} &\textbf{\UnCompilableP} & \textbf{\NonRunnableP} & \textbf{\total}\\ \hline
% \multirow{5}{*}{MagiCoder} & 0                            & 85.3\% (15,701/18,412)            & 9.1\% (247/2,711)          & 21.0\% (568/2,711)            & 14.3\% (388/2,711)   &  44.4\% (1,203/2,711)    \\
% %                           & 0.2                          & 84.8\% (15,965/18,836)            & \multicolumn{1}{c|}{8.9\% (255/2,871)}          & \multicolumn{1}{c|}{22.9\% (658/2,871)}            & 37.5\% (1,076/2,871)          \\
%                            & 0.4                          & 84.2\% (14,751/17,524)            & 9.3\% (259/2,773)          & 23.5\% (653/2,773)            & 14.8\% (404/2,773)   &  47.5\% (1,316/2,773)    \\
%                         & 0.6                          & 84.5\% (12,813/15,155)            & 10.9\%(255/2,342)          & 25.4\% (594/2,342)         & 14.0\% (329/2,342)   &  50.3\% (1178/2,342)    \\
%                            & 0.8                          & 84.6\% (10,403/12,300)            & 12.4\% (235/1,897)          & 26.1\% (496/1,897)            & 14.3\% (272/1,897)   &  52.9\% (1,003/1,897)     \\
%                            & 1.0                          & 85.3\% (7,384/8,658)            & 14.5\% (185/1,274)          & 26.0\% (331/1,274)            & 12.6\% (160/1,274)     &  53.1\% (676/1,274)   \\ \hline
% \multirow{5}{*}{ChatGPT}   & 0                            & 57.3\% (6,708/11,697)            & 4.0\% (199/4,989)          & 32.7\% (1,633/4,989)            & 14.2\% (710/4,989)   &  51.0\% (2,542/4,989)     \\
%                            & 0.4                          & 57.9\% (6,710/11,600)             & 2.6\% (129/4,890)          & 31.9\% (1,558/4,890)            & 15.7\% (769/4,890)    & 50.2\% (2,456/4,890)      \\
%                            & 0.6                          & 56.8\% (6,257/11,013)           & 2.8\% (131/4,756)        & 32.2\% (1,531/4,756)        & 14.2\% (677/4,756)   & 49.2\% (2,339/4,756)      \\
%                            & 0.8                          & 59.2\% (6,666/11,263)            & 4.4\% (202/4,597)          & 30.6\% (1,406/4,597)            & 15.2\% (697/4,597)     & 50.1\% (2,305/4,597)    \\
%                            & 1.0                          & 60.6\% (6,635/10,956)            & 3.2\% (139/4,321)          & 32.9\% (1,420/4,321)            & 14.1\% (611/4,321)     & 50.2\% (2,170/4,321)    \\ \hline
% \end{tabular}
% }
% \end{table}


==> rq4_old.tex <==
\subsection{Results of RQ4}\label{sec:rq4}

\begin{table}[h]
\caption{MagiCoder Task 1 Random Forest Classifier}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Method Exist} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c}{Support} \\ \hline
\multicolumn{1}{c|}{False}        & \multicolumn{1}{c|}{0.95}      & \multicolumn{1}{c|}{0.98}   & \multicolumn{1}{c|}{0.96}     & \multicolumn{1}{c}{18850}   \\
\multicolumn{1}{c|}{True}         & \multicolumn{1}{c|}{0.65}      & \multicolumn{1}{c|}{0.4}    & \multicolumn{1}{c|}{0.49}     & \multicolumn{1}{c}{1696}    \\
\multicolumn{1}{c|}{accuracy}     & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{0.93}     & \multicolumn{1}{c}{20546}   \\
\multicolumn{1}{c|}{macro avg}    & \multicolumn{1}{c|}{0.80}      & \multicolumn{1}{c|}{0.69}   & \multicolumn{1}{c|}{0.73}     & \multicolumn{1}{c}{20546}   \\
\multicolumn{1}{c|}{weighted avg} & \multicolumn{1}{c|}{0.92}      & \multicolumn{1}{c|}{0.93}   & \multicolumn{1}{c|}{0.92}     & \multicolumn{1}{c}{20546}   \\ \hline
                                  &                                &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{Indicator}    & Feature Importance             &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{API Length}   & 0.1852                         &                             &                               &                             \\
\multicolumn{1}{l|}{Confidence}   & 0.2364                         &                             &                               &                             \\
\multicolumn{1}{l|}{PPL}          & 0.3158                         &                             &                               &                             \\
\multicolumn{1}{l|}{Popularity}   & 0.2626                         &                             &                               &          \\  \cline{1-2}                   
\end{tabular}
}
\end{table}

\begin{table}[]
\caption{MagiCoder Task 2 Random Forest Classifier}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Snippet Runnable} & Precision                 & Recall                    & \multicolumn{1}{c|}{F1-score} & Support \\ \hline
\multicolumn{1}{c|}{False}            & \multicolumn{1}{c|}{0.77} & \multicolumn{1}{c|}{0.76} & \multicolumn{1}{c|}{0.77}     & 261     \\
\multicolumn{1}{c|}{True}             & \multicolumn{1}{c|}{0.67} & \multicolumn{1}{c|}{0.67} & \multicolumn{1}{c|}{0.67}     & 184     \\
\multicolumn{1}{c|}{accuracy}         & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{0.73}     & 445     \\
\multicolumn{1}{c|}{macro avg}        & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{0.72}     & 445     \\
\multicolumn{1}{c|}{weighted avg}     & \multicolumn{1}{c|}{0.73} & \multicolumn{1}{c|}{0.73} & \multicolumn{1}{c|}{0.73}     & 445     \\ \hline
                                      &                           &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Indicator}        & Feature Importance        &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Mean Dist}        & 0.3431                    &                           &                               &         \\
\multicolumn{1}{c|}{Max Dist}         & 0.3681                    &                           &                               &         \\
\multicolumn{1}{c|}{Popularity}       & 0.2888                    &                           &                               &         \\  \cline{1-2}
\end{tabular}
}
\end{table}



\begin{table}[]
\caption{ChatGPT Task 1 Random Forest Classifier}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Method Exist} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1-score} & \multicolumn{1}{c}{Support} \\ \hline
\multicolumn{1}{c|}{False}        & \multicolumn{1}{c|}{0.87}      & \multicolumn{1}{c|}{0.92}   & \multicolumn{1}{c|}{0.90}     & \multicolumn{1}{c}{6775}    \\
\multicolumn{1}{c|}{True}         & \multicolumn{1}{c|}{0.68}      & \multicolumn{1}{c|}{0.55}   & \multicolumn{1}{c|}{0.61}     & \multicolumn{1}{c}{2071}    \\
\multicolumn{1}{c|}{accuracy}     & \multicolumn{1}{c|}{}          & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{0.83}     & \multicolumn{1}{c}{8846}    \\
\multicolumn{1}{c|}{macro avg}    & \multicolumn{1}{c|}{0.78}      & \multicolumn{1}{c|}{0.73}   & \multicolumn{1}{c|}{0.75}     & \multicolumn{1}{c}{8846}    \\
\multicolumn{1}{c|}{weighted avg} & \multicolumn{1}{c|}{0.83}      & \multicolumn{1}{c|}{0.83}   & \multicolumn{1}{c|}{0.83}     & \multicolumn{1}{c}{8846}    \\ \hline
                                  &                                &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{Indicator}    & Feature Importance             &                             &                               &                             \\ \cline{1-2}
\multicolumn{1}{l|}{API Length}   & 0.1932                         &                             &                               &                             \\
\multicolumn{1}{l|}{Confidence}   & 0.2704                         &                             &                               &                             \\
\multicolumn{1}{l|}{PPL}          & 0.2612                         &                             &                               &                             \\
\multicolumn{1}{l|}{Popularity}   & 0.2751                         &                             &                               &         \\  \cline{1-2}          
\end{tabular}
}
\end{table}

\begin{table}[]
\caption{ChatGPT Task 2 Random Forest Classifier}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
\hline
\multicolumn{1}{c|}{Snippet Runnable} & Precision                 & Recall                    & \multicolumn{1}{c|}{F1-score} & Support \\ \hline
\multicolumn{1}{c|}{False}            & \multicolumn{1}{c|}{0.65} & \multicolumn{1}{c|}{0.57} & \multicolumn{1}{c|}{0.61}     & 190     \\
\multicolumn{1}{c|}{True}             & \multicolumn{1}{c|}{0.72} & \multicolumn{1}{c|}{0.78} & \multicolumn{1}{c|}{0.75}     & 272     \\
\multicolumn{1}{c|}{accuracy}         & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{}     & \multicolumn{1}{c|}{0.69}     & 462     \\
\multicolumn{1}{c|}{macro avg}        & \multicolumn{1}{c|}{0.68} & \multicolumn{1}{c|}{0.68} & \multicolumn{1}{c|}{0.68}     & 462     \\
\multicolumn{1}{c|}{weighted avg}     & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{0.69}     & 462     \\ \hline
                                      &                           &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Indicator}        & Feature Importance        &                           &                               &         \\ \cline{1-2}
\multicolumn{1}{c|}{Mean Dist}        & 0.3411                    &                           &                               &         \\
\multicolumn{1}{c|}{Max Dist}         & 0.3433                    &                           &                               &         \\
\multicolumn{1}{c|}{Popularity}       & 0.3155                    &                           &                               &         \\  \cline{1-2}
\end{tabular}
}
\end{table}
